Intertwining the Busemann process of the directed polymer model

We study the Busemann process and competition interfaces of the planar directed polymer model with i.i.d.\ weights on the vertices of the planar square lattice, in both the general case and the solvable inverse-gamma case. We prove new regularity properties of the Busemann process without reliance on unproved assumptions on the shape function. For example, each nearest-neighbor Busemann function is strictly monotone and has the same random set of discontinuities in the direction variable. When all Busemann functions on a horizontal line are viewed together, the Busemann process intertwines with an evolution that obeys a version of the geometric Robinson-Schensted-Knuth correspondence. When specialized to the inverse-gamma case, this relationship enables an explicit distributional description: the Busemann function on a nearest-neighbor edge has independent increments in the direction variable, and its distribution comes from an inhomogeneous planar Poisson process. The distribution of the asymptotic competition interface direction of the inverse-gamma polymer is discrete and supported on the Busemann discontinuities which -- unlike in zero-temperature last-passage percolation -- are dense. Further implications follow for the eternal solutions and the failure of the one force -- one solution principle of the discrete stochastic heat equation solved by the polymer partition function.

==> LouisTimoDefs.tex <==

\usepackage{amsmath,amssymb,amsthm,tikz,mathrsfs,mathabx}
\RequirePackage[numbers,sort&compress]{natbib}
\usepackage{scalerel}    %%%%  used first for scaling \bullet for missing argument in a function 
\usepackage{stmaryrd}   %%%% for integer interval notation, though I also have my own    
\usepackage{rotating,centernot,cancel} 
\usepackage{comment,placeins} % added by Louis
\usepackage{mathdots} 
%\usepackage{listofitems} 
%\RequirePackage{listofitems}    %%%%  2022-09-26 for some reason T's attempts to use these packages to handle the \readilst command led to trouble 

%%%%%%%%%%%%%%%%%%%%%%%%%%%% begin added by Erik
\usepackage{stackengine}

\usepackage{mathtools}

\usepackage{xparse}

\usepackage{microtype}

\usepackage{ifthen}

\usepackage{accents}
	\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
	
\def\eps{\varepsilon}
	
% equation shortcuts
% usage: 	\eq{ EQUATIONS }
%		\eeq{ \label{LABEL} EQUATIONS }
%		\eeqs{LABEL}{ EQUATIONS}
\newcommand{\eq}[1]{\begin{align*} #1 \end{align*}}
\newcommand{\eqc}[1]{\begin{gather*} #1 \end{gather*}}
\NewDocumentCommand{\eeq}{om}{\begin{align} \IfNoValueTF{#1}{}{\tag{#1}} \begin{split} #2 \end{split} \end{align}}
\newcommand{\eeqc}[1]{\begin{gather} #1 \end{gather}}
\newcommand{\eeqs}[1]{\begin{align} #1 \end{align}}

%% IF YOU WANT ERIK'S STACK COMMANDS TO WORK AT PARTIAL STRENGTH (ONLY ONE EQUATION NUMBER ALLOWED)
% shortcut for stacking equation references over relations
% usage: 
%\stackref{LABELS SEPARATED BY COMMAS}{SYMBOL} 
%\stackrefp{PHANTOM LABELS}{SYMBOL}
%\stackrefpp{LABELS WANTED}{PHANTOM LABELS}{SYMBOL}
\newcommand{\stackref}[2]{
\stackrel{\mbox{\scriptsize\eqref{#1}}}{#2}
}
\newcommand{\stackrefp}[2]{
%\readlist*\mylist{#1}
\stackrel{\hphantom{\mbox{\scriptsize\eqref{#1}}}}{#2}
}
\newcommand{\stackrefpp}[3]{
%\readlist*\mylist{#1}
%\readlist*\mylistt{#2}
\stackrel{\parbox{\widthof{\scriptsize\eqref{#2}}}{\centering\scriptsize\eqref{#1}}}{#3}
}

%% IF YOU DON"T WANT ANY OF ERIK'S STACK COMMANDS TO WORK
%\newcommand{\stackref}[2]{
%#2
%}
%\newcommand{\stackrefp}[2]{
%#2
%}
%\newcommand{\stackrefpp}[3]{
%#3
%}

%% IF YOU WANT ERIK'S STACK COMMANDS AT FULL STRENGTH (ALLOWING MULTIPLE EQUATION NUMBERS)
%\newcommand{\stackref}[2]{
%\readlist*\mylist{#1}
%\stackrel{\mbox{\scriptsize\foreachitem\x\in\mylist[]{\ifnum\xcnt=1\else,\fi\eqref{\x}}}}{#2}
%}
%\newcommand{\stackrefp}[2]{
%\readlist*\mylist{#1}
%\stackrel{\hphantom{\mbox{\scriptsize\foreachitem\x\in\mylist[]{\ifnum\xcnt=1\else,\fi\eqref{\x}}}}}{#2}
%}
%\newcommand{\stackrefpp}[3]{
%\readlist*\mylist{#1}
%\readlist*\mylistt{#2}
%\stackrel{\parbox{\widthof{\scriptsize\foreachitem\x\in\mylistt[]{\ifnum\xcnt=1\else,\fi\eqref{\x}}}}{\centering\scriptsize\foreachitem\x\in\mylist[]{{\ifnum\xcnt=1\else,\fi\eqref{\x}}}}}{#3}
%}



\newenvironment{proofclaim}[1][Proof]
	{\begin{proof}[#1]}
	{\renewcommand{\qedsymbol}{$\square$ (Claim)}\end{proof}\renewcommand{\qedsymbol}{$\square$}}

% conditional statements (size of delimiter as an optional command)
\newcommand{\givenc}[3][]{#1\{ #2 \: #1| \: #3 #1\}} % with braces
\newcommand{\givenk}[3][]{#1[ #2 \: #1| \: #3 #1]} % with brackets
\newcommand{\givenp}[3][]{#1( #2 \: #1| \: #3 #1)} % with parentheses
\newcommand{\givena}[3][]{#1\langle #2 \: #1| \: #3 #1\rangle} % with angle brackets


\newcommand{\invert}[1]{
           \mathrel{\raisebox{.1em}{
           \reflectbox{\rotatebox[origin=c]{180}{$#1$}}}}}
	
\newcommand{\dd}{\mathrm{d}} % for differentials
\newcommand{\cc}{\mathrm{c}} % for complements

\newcommand{\gs}{\cZ}
\newcommand{\gvv}{\cZ}

\def\H{\mathbb{H}} 

\newcommand{\Asf}{\mathsf{A}}
\newcommand{\Bsf}{\mathsf{B}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\Isf}{\mathsf{I}}
\newcommand{\Gsf}{\mathsf{G}}
\newcommand{\Pscr}{\mathscr{P}}

\newcommand{\ces}{\mathfrak{c}}
\newcommand{\cesm}[2]{\mathfrak{c}_{#2}({#1})}

\newcommand{\ug}{V}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end added by Erik

%\usepackage{newpxmath,newpxtext}
% new \oset macro
\makeatletter
\newcommand{\oset}[3][0ex]{%
	\mathrel{\mathop{#3}\limits^{
			\vbox to#1{\kern-1\ex@
				\hbox{$\scriptstyle#2$}\vss}}}}
\makeatother


%\usepackage[colorlinks]{hyperref}  

\usepackage{graphicx,tikz,subfig,color} %%% ERIK CHANGED SUBFIG TO SUBFIB ON AUGUST 3, 2023
\usetikzlibrary{decorations.pathreplacing}
\usepackage{datetime2}

\RequirePackage{color}
\RequirePackage[colorlinks, urlcolor=my-blue,linkcolor=my-link,citecolor=my-green]{hyperref}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{light-gray}{gray}{0.6}
\definecolor{really-light-gray}{gray}{0.8}

\usepackage{nicefrac}
%\usepackage{enumerate}    %%% make this choice in the main file. 
%\usepackage{wasysym}

%Command to not generate a shitload of files
%\nofiles


%%%%%%%%
\addtolength{\hoffset}{-.8in} 
\addtolength{\textwidth}{1.6in}
\addtolength{\voffset}{-.4in} 
%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
\addtolength{\textheight}{.7in}
%\baselineskip=12pt   %%seems to make no difference? 
\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1


%\newtheorem{theirthm}[theorem]{\sc Theorem} % special environment for referencing theorems of others
%\renewcommand*{\thetheirthm}{\Alph{theirthm}} % this special environment has a separate counter, expressed in letters

\newtheorem{theorem}{\sc Theorem}[section]
\newtheorem{theirthm}[theorem]{\sc Theorem} % special environment for referencing theorems of others
\newtheorem{lemma}[theorem]{\sc Lemma}
\newtheorem{proposition}[theorem]{\sc Proposition}
\newtheorem{corollary}[theorem]{\sc Corollary}
\newtheorem{conjecture}[theorem]{\sc Conjecture}
\newtheorem{claim}[theorem]{\sc Claim}
\newtheorem{assumption}[theorem]{\bf Assumption}
%\newtheorem{definition}[theorem]{\it Definition}
%\newtheorem{remark}[theorem]{\sc Remark}
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{\it Definition}


\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\norm}[1]{\Vert#1\Vert}
\providecommand{\pp}[1]{\langle#1\rangle}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

%%generic definitions 
\def\Coc{\mathscr K}
\def\Cor{\Coc_0}
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cF{\mathcal{F}}   \def\cE{\mathcal{E}}
\def\cG{\mathcal{G}}   \def\cW{\mathcal{W}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cS{\mathcal{S}}  \def\cT{\mathcal{T}}
\def\cI{\mathcal{I}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}  \def\cX{\mathcal{X}}   \def\cY{\mathcal{Y}}
\def\xhat{\hat x}
\def\wg{\eta}
\def\wgtil{\tilde\wg}
\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\gr{\mathcal G}
%\font \mymathbb = bbold10 at 11pt
\def\Hbar{\overline H}
\def\Hhat{\hat H}
\def\Phat{\widehat\P}
\def\Omhat{\widehat\Omega}
\def\kShat{\widehat\kS}
\def\That{\hat T}
\def\Bhat{\hat B}
\def\Vhat{\hat V}
\def\wzhat{\hat\wz}
\def\what{\hat\w}
\def\xbar{\bar x}
\def\t{\mathfrak t}
\def\tmin{{\underline\t}}
\def\tmax{{\bar\t}}

%\newcommand{\one}{{{\rm 1\mkern-2.1mu}\!{\rm I}}}
\newcommand{\one}{\mbox{\mymathbb{1}}}


\def\kS{\mathfrak{S}}

\def\bB{\mathbb{B}}\def\bD{\mathbb{D}}
\def\bE{\mathbb{E}}
\def\bL{\mathbb{L}}
\def\bN{\mathbb{N}}
\def\bP{\mathbb{P}}
\def\bQ{\mathbb{Q}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\Zb{\mathbb{Z}}
\def\bI{\mathbb{I}}

\def\bS{\mathbb{S}}
 \def\Z{\bZ} \def\Q{\bQ} \def\R{\bR}\def\N{\bN}
  \def\avec{\mathbf{a}}     \def\evec{\mathbf{e}}
  \def\svec{\mathbf{s}} \def\tvec{\mathbf{t}} \def\vvec{\mathbf{v}}   
  \def\uvec{\mathbf{u}}
  
  \newcommand{\bfQ}{\mathbf{Q}}
  
% \def\etime{\evec_{\!\scaleobj{0.7}{\nearrow}}} 
 \def\etime{\evec_{\raisebox{3pt}{\scaleobj{0.5}{\pmb\nearrow}}}} 
  \def\espace{\evec^{\raisebox{-2pt}{\scaleobj{0.5}{\pmb\searrow}}}}

\def\ntil{\tilde{n}}
\def\xtil{\tilde{x}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}
\def\qbar{\bar{q}}
\def\Ybar{\overline{Y}}
\def\w{\omega}
\def\om{\omega}
\def\taubar{\bar{\tau}}
\def\omvec{\bar\omega}
\def\psibar{\overline\psi} 
\def\e{\varepsilon}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 
\def\ri{{\mathrm{ri\,}}}

\def\bfx{\mathbf{x}}\def\bfy{\mathbf{y}}\def\bfb{\mathbf{b}}

\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfz}{\mathbf{z}}

\def\mE{\mathbf{E}}   
\def\mH{\mathbf{H}}
\def\mP{\mathbf{P}}
\def\mY{\mathbf{Y}}
\def\m1{\mathbf{1}}
\def\Ustat{\theta}
\def\Vstat{\rho}
\def \sqn{\sqrt{n}}
\def\kS{\mathfrak S}
  \DeclareMathOperator{\refl}{\rho} % reflection of a sequence across the index 0

\DeclareMathOperator{\Var}{Var}   \DeclareMathOperator{\Cov}{Cov}  
%%new def's 
 \def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
 \def\hfun{h}
 \def\cJ{\mathcal{J}}  
 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}   \def\ul{\underline} 
 \def\qvar{\sigma_0}
  \def\chfn{\lambda}  %%char function
 \def\bT{\mathbb{T}} 
 
%%notation specific to this material 
\def\E{\bE}
\def\P{\bP} %% environment measure 
\def\wlev{\omvec} %environment at a level 
\def\shift{\theta}  %spatial shift  
\def\Shift{{\Theta}}  %group of spatial shifts 
\def\shifta{\theta}  %shift  on sequences 
\def\nbhd{\cR}  %set of admissible steps 
\def\jump{v} %jump variable chosen from transition for couplings
\def\flux{H}   %macroscopic flux
\def\vva{v_0} \def\vvb{v_1}   %%%intersections at level j 
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
 
\def\OSP{(\Omega, \kS, \P)}
\def\OS{(\Omega, \kS)}
\def\backpi{\overleftarrow{\pi}} 
\def\backx{\overleftarrow{x}}
%\def\backx{\overset{\leftarrow}{x}}
\def\backX{\overleftarrow{X}}
%\def\backpi{\overset{\leftarrow}{\mathbf{x}}}
\def\Zalt{Z^{\scriptscriptstyle\,\square}}
\def\Zalttil{\wt Z^{\scriptscriptstyle\,\square}}
\def\digamf{\Psi_0} %digamma function 
\def\tmaxigamf{\Psi_1} %trigamma function 
\def\funct lp{L} %a function needed
\def\funct lpbar{\bar L} %a function needed

\def\note#1{{\color{blue}{\bf(}#1{\bf)}}}
\def\New#1{{\color{red}{#1}}}
\def\pfnote#1{{\color{red}{\bf((} #1 {\bf))}}}
%\def\note#1{{\color{nicos-red}{\bf((} #1 {\bf))}}}
%\def\Fnote#1{{\color{orange}{\bf((} #1 {\bf))}}}
\def\timonote#1{{\color{teal}{\bf(}T: #1{\bf)}}}
    \newcounter{eriknotecounter}
    \setcounter{eriknotecounter}{0}
    \newcommand{\eriknote}[1]{%
        \stepcounter{eriknotecounter}%
         {\color{blue}{{\bf(E\theeriknotecounter: } #1}{\bf)}}%
    }

%Firas' notation
\font \mymathbb = bbold10 at 11pt
%\newcommand{\one}{\mbox{\mymathbb{1}}}

\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\Diff{\mathcal D}
\def\EP{\mathcal E}
\def\EPlim{{\widehat{\mathcal E}}}
%\def\G{\mathcal G}
\def\K{\mathcal K}
\def\L{\mathcal L}
\def\cV{\mathcal V}
%\def\Yc{{\check Y}}
\def\Yc{{\w}}
\def\Y{Y}
\def\necorner{{{}_\urcorner}}
\def\swcorner{{{}^\llcorner}}
\def\Xexit{{M^{\cS}}}   %exit point from x-axis
\def\xexit{{m^{\cS}}}   %exit point from x-axis
\def\yexit{{n^{\cW}}}   %exit point from y-axis
%\def\dxexit{{m^{*,\swcorner}}  \def\dyexit{{n^{*,\swcorner}}}    %their duals
\def\xentrance{{m^{\cN}}}   %entrance point to x-boundary
\def\yentrance{{n^{\cE}}}   %entrance point  to y-boundary
\def\rect{{\mathfrak R}}
%\def\gne{G^{\textrm{\tiny{NE}},\xi}}
\def\gne{\wh G^{(\xi)}}
\def\Yh{{\wh\Y}}
\def\gpp{\Lambda}%{{g_{\text{pp}}}}
\def\gpl{{g_{\text{pl}}}}
\def\gppa{\gamma}
\def\Ga{G^{\xi}}
\def\Gsw{G}
%\def\Gne{\wh G}
\def\Ib{I^{\tiny\text{bulk}}}
\def\f{f}
\def\sa{s_{\alpha}}



%Firas' notation
%\def\range{\mathcal R}
%\def\Uset{\mathcal U}
%\def\Dset{\mathcal D}
%\def\G{\mathcal G}
%\def\cA{\mathcal A}
%\def\K{\mathcal K}
%\def\L{\mathcal L}
%\def\Yc{{\check Y}}
%\def\Y{Y}
%\def\necorner{{{}_\urcorner}}
%\def\swcorner{{{}^\llcorner}}
%\def\xexit{{m^{\swcorner}}}   %exit point from x-axis
%\def\yexit{{n^{\swcorner}}}   %exit point from y-axis
%%\def\dxexit{{m^{*,\swcorner}}  \def\dyexit{{n^{*,\swcorner}}}    %their duals
%\def\xentrance{{m^{\necorner}}}   %entrance point to x-boundary
%\def\yentrance{{n^{\necorner}}}   %entrance point  to y-boundary
%\def\rect{{\mathfrak R}}
%\def\V{{V}}
%\def\Vw{V_0}   %%%% the part of the potential that depends only on \w 
\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
\def\cZ{{\mathcal Z}}
%\def\NA{{\mathcal B_0}}
%\def\Zpl{Z}
%\def\Zpp{Z}
%\def\Gpl{G}
%\def\Gpp{G}
%%\def\gpp{g_{\text{\rm pp}}}
%%\def\gpl{g_{\text{\rm pl}}}
%\def\Lapl{\Lambda_{\text{\rm pl}}}
%\def\Lapp{\Lambda_{\text{\rm pp}}}
%\def\ri{{\mathrm{ri\,}}}
%\def\f{{f}} %flux
%%\def\gppa{{\bar g}_{\text{\rm pp}}}
%\def\gppa{{\gamma}}
%\def\amin{{\underline\alpha}}
%\def\amax{{\overline\alpha}}
%\def\nabmin{{\underline\nabla}}
%\def\nabmax{{\overline\nabla}}
%\def\h{{h}}
%\def\hmin{{\underline h}}
%\def\hmax{{\overline h}}
%\def\smin{{\underline s}}
%\def\smax{{\overline s}}
%\def\ximin{{\underline\xi}}
%\def\ximax{{\overline\xi}}
%\def\zetamin{{\underline\zeta}}
%\def\zetamax{{\overline\zeta}}
%
%\def\Bmin{{\underline B}}
%\def\Bmax{{\overline B}}
%\def\Fmin{{\underline F}}
%\def\Fmax{{\overline F}}
%\def\zhat{{\hat z}}
%\def\B{{B}}
%\def\b{{b}}
%\def\Bbar{{\bar\B}}
%\def\cE{{\mathcal E}}
%\def\bB{{\mathbf B}}
%\def\G{{\mathbb G}}
%\def\I{{I}}
%\def\J{{J}}
%\def\Yc{{\w}}
%\def\W{{W}} %%%%  Mai-Pra queueing notation 
%\def\S{{S}}
%\def\A{{A}}
%\def\D{{D}}
%\def\Wp{{\wt W}}
%\def\Sp{{\wt S}}
%\def\Ap{{\wt A}}
%\def\M{{\mathcal M}}
%\def\U{{U}}
%\def\Ombig{{\widehat\Omega}}
%\def\Pbig{{\widehat\P}}
%\def\Ebig{{\widehat\E}}
%\def\kSbig{{\widehat\kS}}
%\def\OBP{(\Omega, \kS, \P)} 
%\def\OBPbig{(\Ombig, \kSbig, \Pbig)} 
%\def\www{{\bar\w}}
%\def\PPP{{\overline\P}}
%\def\EEE{{\overline\E}}
%\def\Ommm{{\overline\Omega}}
\DeclareMathOperator{\extr}{ex}    %%% extreme points of a convex set   

\DeclareMathOperator{\hull}{\overline{\text{co}}}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\bd}{bd}
%\DeclareMathOperator{\extr}{ex}    %%% extreme points of a convex set   

\DeclareMathOperator{\sign}{sign} 
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\var}{Var}
%\DeclareMathOperator{\Var}{Var}
%  \DeclareMathOperator{\Cov}{Cov}  

\DeclareMathOperator{\proj}{Proj}
\DeclareMathOperator{\inter}{int}    %topological  interior  
%\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\aff}{aff}   %affine hull  
\DeclareMathOperator{\effdom}{dom}   %eff domain 
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\kker}{ker}
%\DeclareMathOperator{\refl}{\rho} % reflection of a sequence across the index 0. As MathOperator left too many weird spaces. 
%\DeclareMathOperator{\argmax}{arg max}  %didn't put variable under argmax  

% \newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
%\newcommand{\argmax}[1]{\underset{#1}{\arg\max}\;} 
%\DeclareMathOperator{\argmax}{arg max}  %didn't put variable under argmax  

% \newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
\newcommand{\argmaxa}[1]{\underset{#1}{\arg\max}\;}   %%this one takes an argument underneath 
\newcommand{\argmina}[1]{\underset{#1}{\arg\min}\;} 
\DeclareMathOperator*{\argmax}{arg\,max}   %%
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\supp}{supp}



%\def\O{{\mathcal O}}
%

%%Nicos notation
%\def\Gsw{G^{\rm SW}}
%%\def\Gsw{\overline{G}\!\!\!\!\phantom{G}^{\rm SW}}
%\def\Gne{G^{\rm NE}}   \def\Bne{B^{\rm NE}}
%\def\Ine{I^{\rm NE}}
%\def\Jne{J^{\rm NE}}
%%\def\Ibulk{I^{\rm bulk}}
%\def\Ibulk{I}
%%\def\Jbulk{J^{\rm bulk}}
%\def\Jbulk{J}
%\def\In{I^{\rm N}}
%\def\Jn{J^{\rm N}}
%\def\Ie{I^{\rm E}}
%\def\Je{J^{\rm E}}
%\def\Ge{G^{\rm E}}
%\def\Gn{G^{\rm N}}
%\def\Ine{I^{\rm NE}}
%\def\Jne{J^{\rm NE}}
%%\font\sz=cmr4 at 4pt

%\def\gsw#1{G^{\rm SW, (#1)}}
%\def\gne#1{G^{\rm NE, (#1)}}
%\def\gn#1{G^{\rm N, (#1)}}
%\def\nI#1{I^{\rm N, (#1)}}
%\def\neI#1{I^{\rm NE, (#1)}}
%\def\nJ#1{J^{\rm N, (#1)}}
%\def\neJ#1{J^{\rm NE, (#1)}}
%
%
%%%%%%%%   competition interface  
%\def\cid{\xi_*}
%\def\Bci{B^*}
%\def\Bbarci{\bar B^*}
%%\def\cidm{\cid}
%\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
%\def\cidmax{\overline\xi_*}
%\def\cidd{\tau}   %limit of c.i. 
%\def\wgt{w}

%%%%%Timo
%\def\pp{p}  %the moment hypothesis  
%\def\Ew{m_0}   %mean of \w_0
%\def\opc{\vec p_c} 
%\def\Saset{V}  %the northeast edge of the a-triangle 
%\def\cl{\cO} 
%
%\def\cla{\cO} 
%\def\clb{\cO} 
%\def\aaa{\ell}   %triangle size 
%\def\etamin{{\underline\eta}}
%\def\etamax{{\overline\eta}}
%

\def\pc{\vec p_c}
\def\cO{\mathcal O}

\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to} 
\def\dtoo{\overset{d}\longrightarrow}

%%%%%  from Firas-bultima  
\def\varphimin{\varphi^{{\text\rm{(l)}}}}
\def\varphimax{\varphi^{{\text\rm{(r)}}}}
\def\cidl{\cid^{\text\rm{(l)}}}
\def\cidr{\cid^{\text\rm{(r)}}}
\def\cidlmin{\cidmin^{\text\rm{(l)}}}
\def\cidrmin{\cidmin^{\text\rm{(r)}}}
\def\cidlmax{\cidmax^{\text\rm{(l)}}}
\def\cidrmax{\cidmax^{\text\rm{(r)}}}
\def\cTl{\cT^{\textrm{(l)}}}
\def\thetal{\theta_*^{\text\rm{(l)}}}
\def\thetar{\theta_*^{\text\rm{(r)}}}     
%\def\Bcir{\overline B_*}
%\def\Bcil{\underline B_*}
\def\cT{\mathcal T}

\def\ttvar{\alpha}   %% a variable in a Laplace transform -- not sure what it should be in the end. 

%%%%%%%   Timo def's 2016-09-23 for new file on multiclass CGM  

\def\OFP{(\Omega, \cF, P)} \def\OSP{(\Omega, \kS, \P)}
\def\OSPTh{(\Omega, \kS, \P, \Theta)}
\def\backpi{\overleftarrow{\pi}} 
\def\backx{\overleftarrow{x}}
%\def\backx{\overset{\leftarrow}{x}}
\def\backX{\overleftarrow{X}}
%\def\backpi{\overset{\leftarrow}{\pi}}
\def\Zalt{Z^{\scriptscriptstyle\,\square}}
\def\Zalttil{\wt Z^{\scriptscriptstyle\,\square}}
\def\digamf{\psi_0} %digamma function 
\def\trigamf{\psi_1} %trigamma function 
\def\funct lp{L} %a function needed
\def\funct lpbar{\bar L} %a function needed


\def\Dop{D}    %%% D operator for departure process 
\def\Rop{R}  %% check weights or time in the back of the queue  
\def\Sop{S}    %%% S operator for sojourn time process 
\def\Hop{H}     
\def\Daop{\bfD}   %%n"bigger" operators \def\Daop{\cD}   %%n"bigger" operators 
\def\Haop{\bfH}
\def\Taop{\bfT}
\def\Saop{\bfS} 
%\newcommand{\lzb}{[\![}   %left Z bracket 
%\newcommand{\rzb}{]\!]}   %right Z bracket 
\newcommand{\lzb}{\llbracket}   %left Z bracket 
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\def\bfD{\mathbf D} 
\def\bfH{\mathbf H}
\def\bfS{\mathbf S}
\def\bfT{\mathbf T}

%%%%% scaled objects 

\newcommand\abullet{\hspace{0.9pt}{\raisebox{1pt}{\scaleobj{0.5}{\bullet}}}\hspace{0.9pt}}  %%%% smaller bullet to use inside functions with some space around it 
\newcommand\aabullet{{\tspb\raisebox{1.5pt}{\scaleobj{0.5}{\bullet}}\tspb}}  %%%% bullet to use inside functions, with suitable space around  

\newcommand\bbullet{{\scaleobj{0.7}{\bullet}}} 
\newcommand\rbbullet{{\raisebox{0.9pt}{\scaleobj{0.5}{\bullet}}}}  %good in the superscript of Busemanns  
\newcommand\cbullet{{\scaleobj{0.6}{\bullet}}} 
\newcommand\rcbullet{{\raisebox{1pt}{\scaleobj{0.5}{\bullet}}}} 
\newcommand\rdbullet{{\raisebox{1pt}{\scaleobj{0.4}{\bullet}}}} 

\newcommand\brbullet{{\raisebox{-0.5pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 

\newcommand\bnearrow{{\raisebox{1pt}{\scaleobj{0.6}{\mathbf\nearrow}}}}   %% \nearrow for a superscript so it doesn't look ridiculously big 


\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}

%%%%%%%%%%%%%%  end scaled object 

\def\qedrm{\hfill$\triangle$} 

\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}
 
%\RequirePackage{datetime} %comment out when arxiving or submitting
%\usepackage{filemod}

 \def\Bus{B}
 \def\Buse#1{B^{#1}}
\newcommand\Busv[3]{\overline B^{#1,#2}_{#3}}

\def\Xw{X}  %another letter for a weight 
\def\Yw{W}  %another letter for a weight 
\def\wgtd{\Yw} 
\def\Ywch{\wc\Yw}  %another letter for a weight 
\def\mYw{\mathbf{\Yw}}
 
%\def\caY{\cY^{\bnearrow}}  % a space of ordered n-tuples 
\def\caY{\cY}  % arrow removed to simplify notation. 


%%%%geodesics 
\def\bgeod#1#2{\mathbf b^{#1, #2}}
\def\bgeoda#1{\bgeod{\alpha}{#1}}
\def\bgeodru{\bgeod{\rho}{u}}   \def\bgeodrx{\bgeod{\rho}{x}}   \def\bgeodrz{\bgeod{\rho}{z}}
\def\bgeodr#1{\bgeod{\rho}{#1}}

\def\arrow#1#2{\mathbf a^{#1}_{#2}}
\def\arrowa#1{\arrow{\alpha}{#1}}
\def\arrowru{\arrow{\rho}{u}}   \def\arrowrx{\arrow{\rho}{x}}   \def\arrowrz{\arrow{\rho}{z}}
\def\arrowr#1{\arrow{\rho}{#1}}

\def\counta{\xi}    %%%  count "a",  just a name for a r.v. 

\def\paramb{\tau}   %% needed a parameter -- not sure what a good letter choice is. 

\def\qedex{\hfill$\triangle$}  %%% end of remark, definition and example 

\def\imi{\iota}   %%not sure if want i or \iota for imaginary unit.  imi=imag.i 
\def\imu{\mathbf i}   %% imaginary unit 
%\def\imua{\bold i}      %command \bold obsolete 
\def\imua{\mathbf i}    % Jan. 2016 seems to work the best.



\def\tsp{\hspace{0.5pt}}  %this is sometimes a good spacing in formulas when \, is too large 
\def\tspa{\hspace{0.7pt}}
\def\tspb{\hspace{0.9pt}}\def\tspc{\hspace{1.1pt}}

\def\trng#1#2{#1:#2}    %notation for time range in paths 
\def\parng#1#2{#1\hspace{0.6pt}{\boldsymbol:}\hspace{0.3pt}#2}  %path range 

\def\exUset{\cW}  %exceptional set of directions  
\def\Udiff{\cD}   %directions of differentiability 

\def\pathsp{\mathbb{X}}   %path space   
\def\level{\mathbb L} 
 \def\zevec{\mathbf{0}}  %% origin of R^2 

 
%Boxes for signs 
\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 

%Basis vectors 
\newcommand{\ehat}{\widehat{\evec}}
\newcommand{\et}{\widehat{\evec}_1}   % e_1 + e_2   time 
\newcommand{\etstar}{\et^{\,*}}   %   (e_1 + e_2 )/2 
\newcommand{\ex}{\widehat{\evec}_2}   % e_2 - e_1   space 
\newcommand{\exstar}{\ex^{\,*}}   % (e_2 - e_1)/2  

\def\indep{\ \ \;{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

\def\chdir{\xi}   %most basic char direction 
\def\chdira{\zeta}   \def\chdirb{\eta}   %char directions 
\def\chdirc{\xi}   %char direction coordinate 

\def\brvI{I}    %macros for weights used in describing distributions (bv = Busemann related variables) 
\def\brvJ{J} 
\def\brvX{X} 
\def\brvW{W} 
\def\brvY{Y} 
\def\brvcp{X}   %notation for the coupled process.
\def\brvcpp{Y}   %notation for the second coupled process. 
\def\brvcz{Z} % notation for max of two coupled processes

\def\procX{x} 
\def\procY{y}   %%% more process notation 
\def\procZ{z}

\def\Zpr{Z}   %% another process  

\def\arrX{X}    % symbols for the array 
\def\arrV{V}  
\def\arrZ{Z} 
\def\arrY{Y}  

\newcommand\aUset{\cV^{\tspb\w}} %The set of exceptional directions  

%Geodesics
\newcommand\geo[3]{\boldsymbol{\gamma}_{#1}^{\,#2,\tspa#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geobar[3]{{\overline{\boldsymbol{\gamma}}}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geod[1]{\pi_{#1}} %A generic geodesic without a root or direction. The argument is the index.
%\newcommand\geod[1]{\boldsymbol{\gamma }_{#1}} %A generic geodesic without a root or direction. The argument is the index.

\newcommand\swgeo[3]{\boldsymbol{\sigma}_{#1}^{\,#2,\tspa#3}} %SW Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction

\newcommand\dgeo[3]{\boldsymbol{\gamma}_{#1}^{*,\,#2\!,\,#3}} %dual geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction


\newcommand\geob[3]{\boldsymbol{\rho}_{#1}^{\,#2,\tspa#3}} %Another Geodesic. Arguments are 1.) the index, 2.3.) some symbol, incl.  the starting point, 


%Coalescence points
\newcommand\coal[1]{\mathbf{z}^{#1}} %Coalescence point. The argument is the direction.

%Split points
\newcommand\spt[2]{s_{#1}(#2)}

\def\iff{\Longleftrightarrow}
\def\implies{\Longrightarrow}
\def\rimplies{\Longleftarrow}

\def\Prm{\cN}  %Poisson random measure 
\DeclareMathOperator\BBet{B}  %Beta function 

\def\viiva{\hspace{.7pt}\vert\hspace{.7pt}}
\def\bviiva{\hspace{.7pt}\big\vert\hspace{.7pt}}   %% big viiva, use with \She\bigl( ... \bviiva ... \bigr) 
\def\Bviiva{\hspace{.7pt}\Big\vert\hspace{.7pt}} 
 
\def\Qtree{\mathcal Q}  
\def\Qwalks{\bfQ}  
\def\tiebr{\tvec}   % tiebreaker 

\newcommand\coloneqq{=}     %% trying out getting rid of CS notation  := 


%%%%%%%%%%%%%%%%  definitions from cosz  %%%%%%%%%%%


\newcommand{\cross}{\begin{picture}(12,11)(-2,0)
\put(-9,0){\LARGE$\longrightarrow$}
\put(-1,-2){\LARGE$\downarrow$}  
%\put(-8,-5){\smallskip}
\end{picture}}

\newcommand{\es}[0]{\emptyset}
\newcommand\zarr{z}
\newcommand\zratio{\eta} 
\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\TN}{\ensuremath{\mathbb T_N}}
\newcommand{\TNstar}{\ensuremath{\mathbb T_N^*}}
\newcommand{\SN}[1]{\ensuremath{\mathbb Y_{#1}}}
\newcommand{\SNstar}[1]{\ensuremath{\mathbb Y^{*}_{#1}}}
\newcommand\thetarrr{\hat\theta}  %%theta row - changes in time
\newcommand\thetac{\theta}  %%theta column
\newcommand\thetacv{\theta}  %%theta column vector, the earlier \thetac_{1:N}
\newcommand\thetarrrc{\gamma}  %%theta row column -- both parameters.   %% NOTE: changed from \thetar to avoid conflict with Louis's definitions  

%%%%%%%%%%%%%    end definitions from cosz  %%%%%%%%%%% 

 

